Bicriteria Approximation Algorithms for Priority Matroid Median

Fairness considerations have motivated new clustering problems and algorithms in recent years. In this paper we consider the Priority Matroid Median problem which generalizes the Priority $k$-Median problem that has recently been studied. The input consists of a set of facilities $\mathcal{F}$ and a set of clients $\mathcal{C}$ that lie in a metric space $(\mathcal{F} \cup \mathcal{C},d)$, and a matroid $\mathcal{M}=(\mathcal{F},\mathcal{I})$ over the facilities. In addition each client $j$ has a specified radius $r_j \ge 0$ and each facility $i \in \mathcal{F}$ has an opening cost $f_i$. The goal is to choose a subset $S \subseteq \mathcal{F}$ of facilities to minimize the $\sum_{i \in \mathcal{F}} f_i + \sum_{j \in \mathcal{C}} d(j,S)$ subject to two constraints: (i) $S$ is an independent set in $\mathcal{M}$ (that is $S \in \mathcal{I}$) and (ii) for each client $j$, its distance to an open facility is at most $r_j$ (that is, $d(j,S) \le r_j$). For this problem we describe the first bicriteria $(c_1,c_2)$ approximations for fixed constants $c_1,c_2$: the radius constraints of the clients are violated by at most a factor of $c_1$ and the objective cost is at most $c_2$ times the optimum cost. We also improve the previously known bicriteria approximation for the uniform radius setting ($r_j := L$ $\forall j \in \mathcal{C}$).

==> sections/uni-imp-buggy.tex <==
\subsection{Further improvements}

Observe that the case in which a point $k \in \C$ must travel at most $(6 + 6\epsilon)L$ occurs when $k \in \C_L$ and is assigned to a $j \in \C_T$. In this case, we know that $d(j,k) \leq 2L$. We claim that this distance can be bound tighter.

First, notice that if there is some $j' \in C_L$ such that $d(j',k) \leq 2L$, then assigning $k$ to $j'$, and subsequently using one of $j'$ facilities in the final solution would result in a smaller radius bound. In fact, this would mean that $k$ travels up to $3L$ to reach a facility, which is tight. 

If no such $j'$ exists, then one of two cases can occur. If $d(j,k) > (1 + \epsilon)L$ for all $j \in C_T$, then notice that the ball of radius $L$ around $k$ will be disjoint from any ball of radius $\epsilon L$ that exists around points from $C_T$. If this is the case, we could make $k$ a cluster center, since $k$ exists in a large enough space between other cluster centers to not interfere with disjoint $F'_j$ balls. Filling these spaces by allowing $k$ to be a cluster center will still allow us to construct the half-integral polytope in Stage 2 and proceed with the remainder of the algorithm.

If $d(j,k) \leq (1+\epsilon)L$ for some $j \in C_T$, the $k$ can be assigned to $j$, and we can bound $d(j,k)$ by $(1+\epsilon)L$ instead of $2L$. In doing so, we can show that the farthest any point must travel to reach a center is $(5 + 7 \epsilon)L$. 

We will now show how to derive the $(5 + 7\epsilon)L$ bound. We use the algorithm from this section, but after Filtering we run the following procedure, which intuitively ``fills'' available gaps between points with cluster centers, as described above. 

\begin{algorithm}[ht]
	\caption{$\fillalg$}
	\label{alg:fill}
	\begin{algorithmic}
		\Require Metric $(\F \cup \C,d)$ where $\C = \C_T \cup \C_L$, compatible functions $\phi, \lambda$, updated demands $\a' \in \R^\C$, cluster centers $C = C_T \cup C_L$, $\{D(j) \mid j \in C\}$.  \\
		\State $U \leftarrow \{ k \in \C_L \mid k \notin C \}$ \Comment{All non-cluster center large clients}
		%\State $C \leftarrow \emptyset$ \Comment{The set of cluster centers}
		%\State $\forall j \in \C$ set $a'_j := 0$ \Comment{Initialize new demand variables}
		\While{ $U \neq \emptyset$}
	        \State $\argmin_{k \in U} \phi(k)$
                \State $j \leftarrow j \in C$ s.t. $k \in D(j)$ 
                \If{$\exists j' \in C_L$ s.t. $d(j',k) \leq 2L$}
                \State $D(j) \leftarrow D(j) \setminus \{ k\}$ and $a'_j \leftarrow a'_j - 1$
                \State $D(j') \leftarrow D(j') \cup \{ k\}$ and $a'_{j'}\leftarrow a'_{j'} + 1$
                \State $U \leftarrow U \setminus D(j')$
                \ElsIf{$\exists j' \in C_T$ s.t. $d(j',k) \leq (1+\epsilon)L$}
	        \State $D(j) \leftarrow D(j) \setminus \{ k\}$ and $a'_j \leftarrow a'_j - 1$
                \State $D(j') \leftarrow D(j') \cup \{ k\}$ and $a'_{j'}\leftarrow a'_{j'} + 1$
                \State $U \leftarrow U \setminus \{ k\}$
	     %   \EndFor
                \Else 
                \State $C \leftarrow C \cup \{ k \}$
                \State $D(j) \leftarrow D(j) \setminus \{ k\}$ and $a'_j \leftarrow a'_j - 1$
                \State $D(k) \leftarrow \{ k \}$ and $a'_k = 1$
	        \State $U \leftarrow U \setminus \{ k\}$ 
            \EndIf
		\EndWhile
		\State {\bf Return} updated cluster centers $C$, $\{D(j) : j \in C\}$, demands $\a' \in \Rset^\C$
	\end{algorithmic}
\end{algorithm}

Using the output of $\fillalg$, we will construct the updated instance $\cJ'$, and run the remainder of the algorithm as is. Notice that upon running $\fillalg$, \Cref{fact:filter}(a-c) and (e) still holds. The following are also true. 
\begin{fact}\label{fact:fill}
    After running $\fillalg$ the following will hold. For all $k \in \C_L$ such that $k \notin C$, where $k \in D(j)$ for $j \in C$, (a) if $j \in C_T$, $d(j,k) \leq (1+\epsilon)L$; (b) if $j \in C_L$, $d(j,k) \leq 2L$. 
\end{fact}

Since \Cref{fact:filter}(d) will not hold after running $\fillalg$. For this reason, we need the following claim.

\begin{claim}\label{clm:eps-ck}
    Let $k \in \C$ be assigned to $j \in C$ after $\fillalg$ (i.e. $k \in D(j)$). It will be the case that $\bC_j \leq \bC_k/\epsilon$
\end{claim}

\begin{proof}
    If $k \in \C_T$, then we know that $k$ remains assigned to the cluster center it was assigned to after $\filter$, since $\fillalg$ will only reassign points from $\C_L$. For these points \Cref{fact:filter}(d) still holds, i.e. $\phi(j) \leq \phi(k)$, and hence $\bC_j \leq \bC_k < \bC_k/\epsilon$. This will also be the case for points $k \in \C_L$ that do not get reassigned during $\fillalg$ (i.e. $k \in D(j)$ after $\filter$ and after $\fillalg$). 

    If $k \in \C_L$, and after $\fillalg$ $k$ then there are two cases. If $k$ becomes a cluster center, and the claim trivially holds. Alternatively, $j \in C_L$, and $j$ was not the cluster center $k$ was originally assigned to (i.e. $k \notin D(j)$ after $\filter$). In this case, we know that $\bC_j \leq L$ and $\bC_k > \epsilon L$, hence $\bC_j \leq \bC_k / \epsilon$.  
\end{proof}

Now, we will provide the updated results needed to prove a tighter approximation factor. First, we will show how utilizing $\fillalg$ after filtering and before the remainder of the algorithm increases the cost. In particular, the following two results hold in place of \Cref{lm:cost-filter-uni-imp} and \Cref{thm:cost-uni-imp}.

\begin{lemma}\label{lm:cost-filter-uni-imp2}
The following is true of $\cJ'$. (a) $COST'(x,y) \leq \frac{1}{\epsilon}COST(x,y)$. (b) Any integer solution $(x',y')$ for $\cJ'$ can be converted to an integer solution for $\cJ$ that incurs an additional cost of at most $\frac{2}{\epsilon}\cdot COST(x,y)$. 
\end{lemma}

\begin{proof}
    The proof of (b) is identical to that from the proof of \Cref{lm:cost-filter-uni-imp}. Consider a client $k \in \C \setminus C$ that is relocated to a cluster center $j \in C$ in the new instance. In $COST(x,y)$ client $k$ pays $a_k\bC_k$. In $COST'(x,y)$, the demand of $k$ is moved to $j$ and pays $a_k \bC_j < \frac{a_k}{\epsilon} \bC_k$ where the second inequality follows from \Cref{clm:eps-ck}. Since the facility connection cost remains the same, this means that $COST'(x,y) \leq \frac{1}{\epsilon} COST(x,y)$
\end{proof}

\begin{theorem}
$COST(\tx,\ty) \leq \frac{6}{\epsilon}\cdot COST(x,y)$
\end{theorem}

The proof of the above theorem is identical to that of \Cref{thm:cost-uni} but with updated bounds given by \Cref{lm:cost-filter-uni-imp2}. 

The only update we must make to our radius analysis is to use \Cref{fact:fill} in the proof of \Cref{thm:radius-imp-uni}, which we will formalize below. 

\begin{theorem}
Let $S$ be the output of the aforementioned approximation algorithm for \upmatmed. For all $k \in \C$, $d(k,S) \leq 6L + 6\epsilon L$. 
\end{theorem}

\begin{proof}
Let $k \in D(j)$ after running $\fillalg$. If $k \in \C_L$ and $j \in C_T$, then we have \[ d(k,S) \leq d(j,k) + d(k,S) \leq (1+\epsilon)L + 4L + 6\epsilon L = 5L + 7 \epsilon L.\]

The remaining cases remain identical to those from the proof of \Cref{thm:radius-imp-uni}. 
\end{proof}
